DSPS: Differentiable Stellar Population Synthesis

Models of stellar population synthesis (SPS) are the fundamental tool that relates the physical properties of a galaxy to its spectral energy distribution (SED). In this paper, we present DSPS: a python package for stellar population synthesis. All of the functionality in DSPS is implemented natively in the JAX library for automatic differentiation, and so our predictions for galaxy photometry are fully differentiable, and directly inherit the performance benefits of JAX, including portability onto GPUs. DSPS also implements several novel features, such as i) a flexible empirical model for stellar metallicity that incorporates correlations with stellar age, and ii) support for the diffstar model that provides a physically-motivated connection between the star formation history of a galaxy (SFH) and the mass assembly of its underlying dark matter halo. We detail a set of theoretical techniques for using autodiff to calculate gradients of predictions for galaxy SEDs with respect to SPS parameters that control a range of physical effects, including SFH, stellar metallicity, nebular emission, and dust attenuation. When forward modeling the colors of a synthetic galaxy population, we find that DSPS can provide a factor of 5 speedup over standard SPS codes on a CPU, and a factor of 300-400 on a modern GPU. When coupled with gradient-based techniques for optimization and inference, DSPS makes it practical to conduct expansive likelihood analyses of simulation-based models of the galaxy--halo connection that fully forward model galaxy spectra and photometry.

==> preamble.tex <==
\RequirePackage[normalem]{ulem}
\RequirePackage{color}
\definecolor{RED}{rgb}{1,0,0}
\definecolor{BLUE}{rgb}{0,0,1}
\definecolor{GOLD}{rgb}{1,0.84,0}
\providecommand{\DIFadd}[1]{{\protect\color{teal}\uwave{#1}}}
\providecommand{\DIFdel}[1]{{\protect\color{red}\sout{#1}}}                    
\providecommand{\DIFaddbegin}{}
\providecommand{\DIFaddend}{}
\providecommand{\DIFdelbegin}{}
\providecommand{\DIFdelend}{}
\providecommand{\DIFaddFL}[1]{\DIFadd{#1}}
\providecommand{\DIFdelFL}[1]{\DIFdel{#1}}
\providecommand{\DIFaddbeginFL}{}
\providecommand{\DIFaddendFL}{}
\providecommand{\DIFdelbeginFL}{}
\providecommand{\DIFdelendFL}{}


==> starlife.tex <==
%%%%%%%%%%%%%%
\subsection{Stellar Lifetimes and Remnants}
\label{subsec:starlife}
The lifetime of a star depends sensitively on its initial mass. A massive O star with $\Mstar\gtrsim50\Msun$ will explode as a core-collapse supernova after a few million years, whereas an M star with mass $\Mstar\approx0.1\Msun$ will continue to burn hydrogen for trillions of years, far longer than a Hubble time. Thus at time $\tage$ following some initial burst of star formation, only some fraction of the stars that form continue to survive, $\fsurv(\tage),$ and the remaining mass is returned to the interstellar medium. Due to the mass-dependence of stellar lifetimes, $\fsurv(\tage)$ depends upon the IMF.

In Figure~\ref{fig:msurv_imf}, we show the general behavior of $\fsurv(\tage),$ including its IMF-dependence, which we have calculated using the python-fsps wrapper \citep{python_fsps} of the FSPS library \citep{conroy_gunn_white_2009_fsps1,conroy_gunn_2010_fsps3}. We show results for four different widely-used IMFs: Salpeter \citep{salpeter_1955}, Kroupa \citep{kroupa_etal_1993_imf}, Chabrier \citep{chabrier_2003_imf}, and van Dokkum \citep{van_dokkum_2008_imf}. Each colored curve is accompanied by a dashed curve providing a parametric fit implemented in DSPS; the bottom panel of Figure~\ref{fig:msurv_imf} shows the difference between the fitting function and the result calculated by FSPS; we describe the functional form and parameters used in these fits in Appendix~\ref{sec:msurv}.


%%%%%%%%%%
\begin{figure}
\includegraphics[width=8cm]{Figures/msurv_residual_plot.png}
\caption{{\bf Surviving stellar mass fraction}. For a simple stellar population that formed in a single burst, the quantity plotted on the y-axis, $\fsurv(\tage),$ describes the fraction of the initial mass of the population that survives until the time $\tage$ following the burst. Due to the $\Mstar$-dependence of stellar lifetimes, $\fsurv(\tage)$ depends on the IMF in a manner shown by the different colored curves in the figure. Solid curves show results calculated with the FSPS library; dashed curves show the corresponding fitting function used in DSPS and described in Appendix~\ref{sec:msurv}.}
\label{fig:msurv_imf}
\end{figure}
%%%%%%%%%%

Most stars leave behind a remnant when they die, which is either a white dwarf, a neutron star, or a black hole; the physical nature of the remnant depends on the initial mass of the star. In Figure~\ref{fig:mrem_imf}, we show $\frem(\tage),$ the fraction of stellar mass locked up in remnants, plotted as a function of time for the same four IMFs shown in Figure~\ref{fig:msurv_imf}. Each solid each curve in Figure~\ref{fig:mrem_imf} is accompanied by a dashed curve illustrating a parameterized fitting function for $\frem(\tage);$ we describe the functional form and parameters used in these fits in Appendix~\ref{sec:msurv}.



%%%%%%%%%%
\begin{figure}
\includegraphics[width=8cm]{Figures/mrem_residual_plot.png}
\caption{{\bf Remnant mass fraction}. The quantity $\frem(\tage)$ describes the fraction of the initial mass of a simple stellar population that has been transformed into stellar remnants at the time $\tage.$ As in Figure~\ref{fig:msurv_imf}, different colored curves show results for different assumed IMFs as indicated in the legend; solid curves show results derived with FSPS; dashed curves show the corresponding fitting functions used by DSPS and described in Appendix~\ref{sec:msurv}. \aph{I plan to work on this a little more to get a slightly better fit.}}
\label{fig:mrem_imf}
\end{figure}
%%%%%%%%%%


